Leveraging energy storage to optimize data center electricity cost in emerging power markets

Energy storage in data centers has mainly been used as devices to backup generators during power outages. Recently, there has been a growing interest in using energy storage devices to actively shape power consumption in data centers to reduce their skyrocketing electricity bills. In this paper, we consider using energy storage in data centers for two applications in a joint fashion: reducing peak demand charges and enabling data centers to participate in regulation markets. We develop an optimization framework that captures the cost of electricity, degradation of energy storage devices, as well as the benefit from regulation markets. Under this frame- work, using real data Microsoft data center traces and PJM regulation signals, we show the electricity bill of a data center can be reduced by up to 20%. Furthermore, we demonstrate that the saving from joint optimization can be even larger than the sum of individually optimizing each component. We quantify the particular aspects of data center load profiles that lead to this superlinear gain. Compared to prior works that consider using energy storage devices for each single application alone, our results suggest that energy storage in data centers can have much larger impacts than previously thought possible.

==> simple_control.tex <==
In this section, we introduce the simulation method to
solve for the optimization problem we proposed before. 
The main purpose of this paper is to define the "non-linear saving" phenomenon of doing RS and PS
at the same time and to investigate why this extra benefit happens. Therefore, instead of using some complicated online control algorithms, we consider a simple control policty in this paper.

\subsection{A deterministic method to decide the regulation capacity}

Review the general optimization problem we have in section II.
\begin{equation}\label{Sec:P3:1}
\begin{aligned}
& \underset{C, b(t)}{\text{min}}
& &  \lambda_{elec} \sum_{t=1}^{T} {[s(t)-b(t)]} + \lambda_{peak} \underset{t=1...T}{\text{max}}{[s(t)-b(t)]}\\
& & &+ \lambda_d \sum_{t=1}^{T} {|b(t)|} \\
& & &-(\lambda_c \* C- \lambda_r \sum_{t=1}^{T}{|-s(t)+b(t)+y(t)-Cr(t)|})\\
& & & \\
& \text{s.t.} & &  C \geq 0 \\
& & &  y(t) = s(t) \\
& & &  -P \leq b(t) \leq P \\
& & &  SoC_{min} \leq \frac{SoC_{ini} \* E + \sum_{t=1}^{t}b(\tau) \* t_s}{E} \leq SoC_{max} \\
\end{aligned}
\end{equation}

If we set $\lambda_{peak}=0$, we recover to the optimize battery usage for regulation service problem.  
If we set the regulation term $-(\lambda_c \* C- \lambda_r \sum_{t=1}^{T}{|-s(t)+b(t)+y(t)-Cr(t)|})$ to $0$, 
we could recover to using battery usage for peak shaving case. So equation (\ref{Sec:P3:1}) represents the 
general optimization problem trying to solve.

To determine the regulation capacity $C$, we assume that $r(t)$ is known and solve the optimization problem 
in a deterministic way. And then we will use the optimal $C^{*}$ as the bidded regulation capacity sent to the 
market operator. As we mentioned before, $r(t)$ is a random signal and hard to predict. According to the statistics
of r(t)\footnote[1]{Data from RegD signal, PJM, 2013.06-2014.05} in \todo{Fig. \ref{Fig:P3:1}, we found it generally obeys a Gaussian distribution with higher possibility at $-1$ and $1$}. 

\subsection{Battery control policy}

\todo{...}

\subsection{Simple control algorithm}

Provide algorithm here 
\begin{center}
	\begin{tabular}{l}
		\hline
		\textbf{Simple control algorithm for (\ref{Sec:P3:1})}\\
		\hline
		1. Solve the deterministic optimization problem, get $C^{*}$ \\ 
		
		2. ....\\
		
		\vspace{36pt}
		
		3. ....\\
		\hline
	\end{tabular}
\end{center}
